VEIGAR: View-consistent Explicit Inpainting and Geometry Alignment for 3D object Removal

Recent advances in Novel View Synthesis (NVS) and 3D generation have significantly improved editing tasks, with a primary emphasis on maintaining cross-view consistency throughout the generative process. Contemporary methods typically address this challenge using a dual-strategy framework: performing consistent 2D inpainting across all views guided by embedded priors either explicitly in pixel space or implicitly in latent space; and conducting 3D reconstruction with additional consistency guidance. Previous strategies, in particular, often require an initial 3D reconstruction phase to establish geometric structure, introducing considerable computational overhead. Even with the added cost, the resulting reconstruction quality often remains suboptimal. In this paper, we present VEIGAR, a computationally efficient framework that outperforms existing methods without relying on an initial reconstruction phase. VEIGAR leverages a lightweight foundation model to reliably align priors explicitly in the pixel space. In addition, we introduce a novel supervision strategy based on scale-invariant depth loss, which removes the need for traditional scale-and-shift operations in monocular depth regularization. Through extensive experimentation, VEIGAR establishes a new state-of-the-art benchmark in reconstruction quality and cross-view consistency, while achieving a threefold reduction in training time compared to the fastest existing method, highlighting its superior balance of efficiency and effectiveness.

==> introduction/introduction_new.tex <==
Novel View Synthesis (NVS) and 3D generation have recently achieved substantial progress, particularly in editing tasks \cite{mildenhall2020nerf, kerbl3Dgaussians}. While early approaches based on 2D inpainting \cite{pathak2016context, iizuka2017globally, yu2018generative, liu2018image, suvorov2022resolution} often suffer from cross-view inconsistencies, recent efforts such as SPIn-NeRF \cite{spinnerf} and SDS-based approaches \cite{alldieck2024score, bahmani2024fourdfy, yang2024semantic, poole2023dreamfusion, Liang_2024_CVPR} attempt to promote scene-level consistency through global supervision. However, these methods primarily focus on latent-space alignment, leaving pixel-space correspondence underconstrained. Moreover, they often rely on accurate metric depths, requiring a computationally expensive 3D reconstruction stage that introduces additional overhead and potential inaccuracies. Recent cross-view attention methods \cite{huang2025_2502.11801, shi2024crossview, gaussctrl2024, chen2023gaussianeditor, salimi2025geometry, cerkezi2023multi, cao2024mvinpainter} alleviate spatial inconsistencies, but the reliance on approximate depth fields or feature space matching still limits full pixel-level coherence.

To address these challenges, we propose \textbf{S3DI}, a novel framework that enables explicit pixel-space alignment for 3D editing. Our method leverages deep stereo depth predictions to enable robust cross-view projections without requiring dense metric depths, thereby bypassing the need for pretraining heavy radiance field models. To further enhance projection reliability, we reformulate the problem as the optimization of a low-dimensional parameter set instead of predicting dense depths, simplifying the process while improving robustness. Additionally, we introduce a scale-invariant depth loss integrated into the reconstruction stage, which not only removes the need for per-view scale and offset calibration, but also maintains geometric consistency throughout the entire reconstruction process, beyond merely initial structure formation. Extensive experiments demonstrate that S3DI simplifies the 3D editing pipeline while achieving superior performance in novel view synthesis and object removal, establishing a promising new direction for efficient and consistent 3D inpainting.


==> method/method1.tex <==
\paragraph{Depth-based Projection} Given a known camera intrinsic $\mathbf{K}$ and a metric depth map, which can be obtained through Multiview Stereo Depth (MVS) or reconstruction techniques, the corresponding pixel $\mathbf{p'}$ in the target view can be computed by projecting $\mathbf{p}$ from the reference view as:

\begin{equation}
\mathbf{p}' = F_{\mathbf{K}, \mathbf{R}, \mathbf{t}}(\mathbf{p}, d(\mathbf{p})),
\end{equation}

where $F$ denotes the projection function parameterized by the intrinsics $\mathbf{K}$, and $\mathbf{R}$ and $\mathbf{t}$ represent the relative rotation and translation from the anchor view to the target view. Specifically, $F$ lifts the pixel coordinate $\mathbf{p}$ into 3D space using the estimated depth $d(\mathbf{p})$, applies the rigid transformation $(\mathbf{R}, \mathbf{t})$, and reprojects the transformed point back to the image plane using $\mathbf{K}$. The explicit expressions for this projection can be formulated in Eq. \ref{eq:project}.

A key characteristic of Deep Stereo Depth (DSD) is its ability to rapidly generate consistent depth maps across multiple views. While DSD does not provide metric depth values for each view, it guarantees global geometry matching between depth maps with an unknown scale factor. Under this assumption, we propose that the pixel $\mathbf{p}$ from the anchor view can be lifted to the reference view via an alternative projection:

\begin{equation}
\mathbf{p}' = F_{\tilde{\mathbf{K}}, \mathbf{R}, \mathbf{t}}(\mathbf{p}, D(\mathbf{p})),
\end{equation}

where the depth map $D(\mathbf{p})$ is estimated by DSD at a pixel $\mathbf{p}$, and $\tilde{\mathbf{K}}$ is an implicit intrinsic parameter. In practice, $\tilde{\mathbf{K}}$ is an unknown matrix \( \tilde{\mathbf{K}} \in \mathbb{R}^{3 \times 3} \), while a sparse version of the metric depth map, $d(\mathbf{p})$, can be directly obtained from Structure-from-Motion (SfM). Instead of fully recovering the dense metric depth, we focus on estimating the low-dimensional $\tilde{\mathbf{K}}$, which offers a more efficient and stable solution. The implicit intrinsics $\tilde{\mathbf{K}}$ can be recovered by minimizing the discrepancy between the projections produced by the DSD-predicted depths and those generated from the known quantities:

\begin{equation}
F_{\tilde{\mathbf{K}}, \mathbf{R}, \mathbf{t}}(\mathbf{p}, d(\mathbf{p})) \sim F_{\mathbf{K}, \mathbf{R}, \mathbf{t}}(\mathbf{p}, D(\mathbf{p})),
\end{equation}

where $\sim$ denotes equality up to an unknown global scale factor, reflecting the inherent scale ambiguity in DSD outputs. 

We employ DUST3R \cite{dust3r} to predict the estimated depth maps \( D(\mathbf{p}) \), and then leverage point clouds obtained from SfM to infer the corresponding sparse metric depths \( d(\mathbf{p}) \) through projection. To estimate the implicit camera intrinsic matrix \( \tilde{\mathbf{K}} \), we perform two projections on the sparse correspondences to calculate the discrepancies, which are then minimized using least-squares optimization. After obtaining a robust estimate of \( \tilde{\mathbf{K}} \), we project the anchor image to other views using the estimated depth information, preparing for the subsequent inpainting phase.

By aligning these depth values, we enable the projection of the anchor image from the source camera pose into a target view using the transformed DSD depth as follows:
\begin{equation}
\mathbf{p}' = F_{\mathbf{K}, \mathbf{R}, \mathbf{t}}(\mathbf{p}, \tilde{D}(\mathbf{p})),
\end{equation}
where $\mathbf{K}$ denotes the calibrated intrinsic matrix, and $\mathbf{R}, \mathbf{t}$ represent the relative pose between the source and target views. The term $\tilde{D}(\mathbf{p})$ denotes the transformed depth map, aligned to the metric scale of the target coordinate system.

As Deep Stereo Depth (DSD) methods provide only an implicit pixel-to-scene relationship without metric scale, we aim to convert the lifted 3D coordinates from the DSD representation into a known metric coordinate system defined by calibrated camera intrinsics. To achieve this, we leverage an initial sparse reconstruction obtained from Structure-from-Motion (SfM), which provides intrinsic parameters $\mathbf{K}$ and a sparse point cloud with accurate metric depth. We transform the dense depth predictions from DSD into this coordinate system by adapting them to the SfM-derived sparse depth.

Specifically, we project the SfM point cloud into the anchor camera pose to obtain a sparse metric depth map, which serves as a supervisory signal. We then minimize the discrepancy between this sparse ground truth and the DSD-predicted depth values. This conversion process is optimized using an $\mathcal{L}_{2}$ loss:

\begin{equation}
\mathcal{L}_{\text{trans}} = \sum_{\mathbf{p} \in \mathcal{M}}(d(\mathbf{p}) - D(\mathbf{p}) )^2,
\end{equation}

where $d(\mathbf{p})$ is the sparse metric depth obtained from SfM and $D(\mathbf{p})$ is the corresponding DSD-predicted depth.

While converting a dense depth map to a metric-consistent representation may initially appear complex, we observe that the underlying optimization is effectively equivalent to estimating a low-dimensional implicit camera intrinsic matrix $\mathbf{K}'$ for an alternative projection formulation. Consequently, this task can be efficiently addressed using another lightweight neural network, enabling stable and scalable alignment between DSD-predicted depths and metric geometry.


==> preliminaries/DSD.tex <==
Multiview stereo depth estimators aim to produce a cross-view scale-consistent depth map by incorporating information from multiple images. Classical Multi-View Stereo (MVS) methods achieve this by projecting pixels from a reference view to source views using known camera parameters and hypothesized depths \cite{mvsnet}. The projection of a pixel $\mathbf{p}$ at depth $d$ follows:
\begin{equation}
\mathbf{p}_i(d) = \mathbf{K}_i \left( \mathbf{R}_i \mathbf{R}_0^\top (\mathbf{K}_0^{-1} \mathbf{p} \cdot d) - \mathbf{R}_i \mathbf{R}_0^\top \mathbf{t}_0 + \mathbf{t}_i \right),
\label{eq:project}
\end{equation}
where $\mathbf{K}_0$, $\mathbf{K}_i$ are intrinsics, and $\mathbf{R}_0$, $\mathbf{t}_0$, $\mathbf{R}_i$, $\mathbf{t}_i$ denote extrinsics of reference and source views. This warping enables construction of a cost volume to infer depth. However, MVS pipelines are often computationally heavy and sensitive to textureless or occluded regions \cite{casmvsnet, patchmatchnet}.

In contrast, deep stereo depth (DSD) estimation directly predicts depth or disparity maps from image pairs via neural networks \cite{mccnn, gcnet, ganet-cvpr2022, Wang_2024_CVPR, ye2025no}. Rather than relying on explicit geometric projections, DSD models learn implicit pixel-scene relationships from data. Although this implicit modeling sacrifices direct pixel-world alignment, it maintains view-consistent geometry and offers significantly faster inference compared to traditional MVS approaches \cite{hitnet, deeppruner, acvnet}. This efficiency makes DSD methods particularly suitable for real-time or large-scale 3D applications.

